Combining expert knowledge and neural networks to model environmental stresses in agriculture

In this work we combine representation learning capabilities of neural network with agricultural knowledge from experts to model environmental heat and drought stresses. We first design deterministic expert models which serve as a benchmark and inform the design of flexible neural-network architectures. Finally, a sensitivity analysis of the latter allows a clustering of hybrids into susceptible and resistant ones.

==> material/target_journals.tex <==
BMC Bioinformatics (IF: 2.3)
    - Anne-Katrin hat hier schon veröffentlicht und meinte der Scope wäre passend



Bioinformatics (IF 4.5)
    - Anne-Katrin meinte, dass die Daten hier nicht super passend sind, daher vermutlich keine gute Option



Computers and Electronics in Agriculture (IF 3.1)



Plos One (2.7)



Frontiers in Plant Science (4.3)
    - Dies wurden uns von dem serbischem Team empfohlen
    


BMC Biodata Mining
    -[https://biodatamining.biomedcentral.com/]



Environmental Modelling & Software     
    -[https://www.journals.elsevier.com/environmental-modelling-and-software]

 


Ecological Modelling
    - https://www.journals.elsevier.com/ecological-modelling

 

Field Crops Research
    - https://www.journals.elsevier.com/field-crops-research


